Software Reconfiguration in Robotics

Robots often need to be reconfigurable$-$to customize, calibrate, or optimize robots operating in varying environments with different hardware). A particular challenge in robotics is the automated and dynamic reconfiguration to load and unload software components, as well as parameterizing them. Over the last decades, a large variety of software reconfiguration techniques has been presented in the literature, many specifically for robotics systems. Also many robotics frameworks support reconfiguration. Unfortunately, there is a lack of empirical data on the actual use of reconfiguration techniques in real robotics projects and on their realization in robotics frameworks. To advance reconfiguration techniques and support their adoption, we need to improve our empirical understanding of them in practice. We present a study of automated reconfiguration at runtime in the robotics domain. We determine the state-of-the art by reviewing 78 relevant publications on reconfiguration. We determine the state-of-practice by analyzing how four major robotics frameworks support reconfiguration, and how reconfiguration is realized in 48 robotics (sub-)systems. We contribute a detailed analysis of the design space of reconfiguration techniques. We identify trends and research gaps. Our results show a significant discrepancy between the state-of-the-art and the state-of-practice. While the scientific community focuses on complex structural reconfiguration, only parameter reconfiguration is widely used in practice. Our results support practitioners to realize reconfiguration in robotics systems, as well as they support researchers and tool builders to create more effective reconfiguration techniques that are adopted in practice.

==> Makefile <==
TEX=*.tex

BIB=*.bib

IMGS=figures/*.pdf

main.pdf: $(TEX) $(BIB) $(IMGS)
	pdflatex main.tex &&\
	bibtex   main &&\
	pdflatex main && \
	pdflatex main

cr: main.pdf
	embedfonts main.pdf 

clean: 
	rm -f *~ *.aux *.bbl *.bbg *.log *.orig *.log main.pdf *.blg; find .. -type f -name '*~' -o -name '*.bak' -o -name 'Rplots.pdf' -o -name '*.backup' -o -name '*.orig' | xargs rm -f 
         
	


==> sections/related.tex <==
\section{Related Work}
\label{sec:related}
%In this work, we focus on software recofinguration in robotics.
%\paragraph{Adaptability}
%The ability of the system to adapt itself to different work scenarios, different environments and conditions.
%Adaptation may take place over long or short time scales. It may relate to local control systems or actions, or to the whole system or to interaction.
%
%Adaptability implies that the system performs optimisation against some performance criteria. This requires defined performance metrics that can be used to drive the adaptation process.
%Adaptability can be applied many different aspects of a robot system:
%\begin{itemize}
%	\item Adaptation of sensor processing to account for different environmental conditions, for example a vision sensor adapting to a failed sensing element.
%	\item The control parameters of a controller adapting to account for changes in the specific properties of an actuator (increased friction, reduced power etc.).
%	\item Adaptation of the intrinsic and extrinsic parameters of sensor configuration as they change over time due to wear and tear
%	\item The adaptation to a new environment with respect to the strategy used to achieve a function. For example adapting a cleaning scan pattern to optimise time in a room after examining performance metrics.
%\end{itemize}
%
%Adaptability must be clearly distinguished from Configurability and Decisional Autonomy.
%Adaptability involves the altering of parameters over time based on experience with the goal of optimising performance.
In the robotics domain, the term \emph{reconfiguration} is mostly used to describe the ability to change the physical structure of a robot, usually including reconfiguration on the software level on which we focus.
In the last 30 years, several surveys have been published on three classes of reconfigurable systems, namely (i) robots composed of multiple identical modules, (ii) robots composed of modules with specialized functionalities, and (iii) swarms of mobile robots.

Robots composed of multiple identical modules can be mechanically assembled to different physical shapes (e.g., a snake) and can reconfigure their shape for adapting to environments~\citep{Dudek1993,Yim2007,Moubarak2012,Ahmadzadeh2015,Chennareddy2017,Alattas2018}.
Robots composed of modules with specialized functionalities can reconfigure to perform different tasks \citep{Liu2016}.
Swarms of mobile robots (e.g., swarms of UAVs) can reconfigure the topology resulting from coalition formation during cooperative task execution~\citep{Abukhalil2015,Shlyakhov2017}.

 \edit{As discussed in the introduction,  adaptability is a concept related to reconfigurability, but with important differences. Adaption exclusively describes a behavior, which is changed for, e.g., optimizing some quality aspect, dealing with specific characteristics of the operational environment, etc. Instead, reconfiguration concerns the modification of the system state or configuration, even from the physical or structural point of view. In some cases a reconfiguration can alter the system behaviour and can be even be performed at runtime. Because of that the two concepts can be confused. However, a reconfigurable system not necessarily is self-adaptive, and vice versa.
Concerning adaptative and self-adaptive systems (SAS), we can find a number of survey papers aiming at providing a taxonomy of SASs
and identifying the most important research gaps~\cite{Salehie2009,Krupitzer2015}.  Salehie and Tahvildari~\cite{Salehie2009} also provide a taxonomy of self-adaptation, including the object to adapt, realization issues, temporal characteristics, and interaction concerns. 
Krupitzer et al.~\cite{Krupitzer2015} presents a taxonomy of self-adaptation and a survey on engineering SASs. The work in~\cite{MACIASESCRIVA20137267} reviews the state of the art on self-adaptivity from the computer sciences and cybernetics points of view.
Puviani et al. propose a classification of self-adaptation patterns that support self-adaptation at the component level and the system level~\cite{Zambonelli2013}. Hezavehi et al.~\cite{Hezavehi2021}  discuss how the concept of uncertainty is understood in the community, together with an understanding of how uncertainty is currently handled in the engineering of self-adaptive systems.
Finally, a recent book provides a historical perspective of SASs~\cite{Weynsbook}. The book organizes the history of SASs in seven waves focusing on complementary aspects of engineering self-adaptive systems, i.e. automating tasks, architecture-based adaptation, runtime models, requirements-driven adaptation, guarantees under uncertainties, control-based software adaptation, and learning from experience.
Instead, in this work we aim at describing the state of the art and state of practice in software reconfiguration in robotics.
}


%Two secondary studies are specifically relevant for our investigation because they provide taxonomies of reconfigurable robotic systems and clarify the terminology used in the literature.
%%\ugh{we proposed the definition that a DRS is a system whose subsystems can be
	%%modified or have their configurations changed during operation to reach a certain
	%%goal.} This definition is similar to the definition proposed by others papers \ugh{[xx54, xx37]}
%%and also encompasses the concept of reconfigurable computing
%More specifically, a Dynamic Reconfigurable System is defined as ``\emph{a system whose subsystems can be modified or have their configurations changed during operation; dynamic reconfiguration enables real-time systems adaptation}''~\citep{Fornari2019}. The paper provides several examples of reconfigurable robotic systems and focus on two aspects that were not analyzed in previous studies: the reconfiguration of the computing hardware (mostly FPGAs) and, although only marginally, the reconfiguration of the robot control system (e.g. the autonomous navigation system).
%
%
%Tan et al.~\citep{Tan2020} define reconfigurable systems as ``\emph{those that can reversibly achieve distinct configurations or states via alternating system form or function to achieve the desired outcome within acceptable reconfiguration time and cost.}''
%In this paper, self-reconfigurable robots are described as ``\emph{machines that can change their morphologies as per prescribed requirement or are adaptable to the environments with provided level of autonomy.}''
%In turn, autonomous reconfigurability is described as ``\emph{The extent to which a self-reconfigurable robot can sense its environment, plan its configuration based on that environment, and act to transform into specific configurations upon that environment with the intent of achieving some goal (either given by human or created by the robot itself).}''
%To achieve such reconfiguration, robots require the mechanism of reconfigurability, described in the paper as ``\emph{the extent/degree to which a self-reconfigurable robot or robotic systems can transform and evolve to another meaningful configuration with a certain degree of autonomy or human intervention.}''

Several secondary studies focus on the hardware reconfiguration of various types of robotic systems.
These include self-reconfigurable industrial robots~\citep{Setchi2004} and modular mobile robots~\citep{Liu2016, Chennareddy2017}.
They mostly cover aspects related to the mechanical morphology of reconfigurable robots.
A few papers review techniques and algorithms for controlling reconfigurable robots~\citep{Ahmadzadeh2015, Tan2020}.
Swarm robotics is a special category of reconfigurable systems, where reconfiguration is changing the swarm aggregation topology of many identical autonomous robots~\citep{Dudek1993}.

To the best of our knowledge, only one secondary study mentions software aspects of robot reconfiguration~\citep{Fornari2019} and presents an SLR that investigates how different kinds of dynamically reconfigurable systems are classified and what are their definitions.
It mentions UAV robots, but does not focus on robotics specifically.

%Garcia et al.~
\cite{GarciaEMSE2022} present a multiple-case study to compare the state of practice with the state-of-the-art in software variability in service robotics.
It does not focus on software reconfiguration specifically, but highlights a pressing challenge to make robots using generic configurations work robustly in most expected contexts without major tuning.
Thus, this work testifies to the importance of an in-depth study on software reconfiguration in robotics.

